Large-Scale Simulation of Quantum Computational Chemistry on a New Sunway Supercomputer

Quantum computational chemistry (QCC) is the use of quantum computers to solve problems in computational quantum chemistry. We develop a high performance variational quantum eigensolver (VQE) simulator for simulating quantum computational chemistry problems on a new Sunway supercomputer. The major innovations include: (1) a Matrix Product State (MPS) based VQE simulator to reduce the amount of memory needed and increase the simulation efficiency; (2) a combination of the Density Matrix Embedding Theory with the MPS-based VQE simulator to further extend the simulation range; (3) A three-level parallelization scheme to scale up to 20 million cores; (4) Usage of the Julia script language as the main programming language, which both makes the programming easier and enables cutting edge performance as native C or Fortran; (5) Study of real chemistry systems based on the VQE simulator, achieving nearly linearly strong and weak scaling. Our simulation demonstrates the power of VQE for large quantum chemistry systems, thus paves the way for large-scale VQE experiments on near-term quantum computers.

==> Makefile <==
base_name := Manuscript
datestamp := $(shell date +"%Y-%m-%d")
workdir   := $(shell basename $(shell pwd))


%.pdf: %.tex
	pdflatex --interaction=nonstopmode $<
	bibtex $*.aux
	pdflatex --interaction=nonstopmode $<
	pdflatex --interaction=nonstopmode $<


all: $(base_name).pdf  
	(evince $(base_name).pdf  &)


$(base_name).pdf: $(base_name).tex $(base_name).bib 

figures:
	$(MAKE) -C figures

dated:
	[ ! -d archive ] && mkdir archive
	$(MAKE) pdf
	cp -a $(base_name).pdf archive/$(base_name)-$(datestamp).pdf

tgz:
	$(MAKE) clean
	cd .. && tar -zcvf $(base_name)-$(datestamp).tgz $(workdir)

backup:
	$(MAKE) tgz
	cd .. && rsync -avizP $(base_name)-$(datestamp).tgz barin:backup/.

semiclean:
	rm -f *~ *.aux *.bbl *.blg *.brf *.bmt *.dvi *.log *.toc \
	$(base_name).pdf $(base_name).ps $(base_name).out $(base_name)Notes.bib

figuresclean:
	$(MAKE) -C figures clean

clean:
	$(MAKE) semiclean

.PHONY: clean figuresclean semiclean backup

